Design-based Estimation Theory for Complex Experiments

This paper considers the estimation of treatment effects in randomized experiments with complex experimental designs, including cases with interference between units. We develop a design-based estimation theory for arbitrary experimental designs. Our theory facilitates the analysis of many design-estimator pairs that researchers commonly employ in practice and provide procedures to consistently estimate asymptotic variance bounds. We propose new classes of estimators with favorable asymptotic properties from a design-based point of view. In addition, we propose a scalar measure of experimental complexity which can be linked to the design-based variance of the estimators. We demonstrate the performance of our estimators using simulated datasets based on an actual network experiment studying the effect of social networks on insurance adoptions.

==> Text/check_list.tex <==
Lemma 1: checked May 6
Lemma 2: checked May 6
Lemma 3: checked May 6
Lemma 4: checked May 6
Lemma 5: checked May 6
Lemma 6: checked May 6
Lemma 7: checked May 6
Lemma 8: checked May 6
Lemma 9: checked May 6
Lemma 10: checked May 6
Lemma 11: chekced May 6
Lemma 12: checked May 6
Lemma 13: checked May 7
Lemma 14: checked May 7
Lemma 15: checked May 7
Lemma 16: checked May 7


Theorem 1: checked May 6
Corollary 1: checked May 6

Theorem 2: checked May 6


Lemma 2: checked May 6
Theorem 3: checked May 6 
Theorem 4: checked May 7
Theorem 5: checked May 7
Theorem 6: 


==> Text/old_optimal_GR.tex <==


%%%%%%OLD WRITINGS FOR OPTIMAL GR ESTIMATOR%%%%%%%
QMLE-GR estimators and No-harm-GR estimators both elicit $\theta_n$ from other criteria. Instead of requiring $\theta_n$ to be the maximizer of a pseudo-likelihood, we can choose $\theta_n$ to directly minimize the implied asymptotic variances. That is, we define 
\begin{equation}\label{optimal-gr}
    \theta_n\equiv\arg\min_{\theta\in \Theta}  \frac{1}{n^2}c' \onesmat'\diag(y-f(\theta))\hspace{1pt}\dmat\hspace{1pt} \diag(y-f(\theta))\onesmat c.\footnote{In theory, there is a possibility that even the minimized asymptotic variance may be larger than that of the IPW estimator $\frac{1}{n^2} c' \onesmat'\diag(y)\hspace{1pt}\dmat\hspace{1pt} \diag(y)\onesmat c$. This will not happen if the imputation functions can impute the $\0_{kn}$ vector (i.e., $\0_{kn}\in \{f(\theta)\}_{\theta\in\Theta}$) or if the $\dmat$ matrix nullifies the intercept matrix $\dmat\onesmat=\0_{kn\times k}$ and, for each arm, the imputation functions can impute the same potential outcomes for each unit. If neither condition is satisfied and 0 is in the parameter set $\Theta$, one can guarantee no harm by shifting the parameter set by $f(0)$ and define $\theta_n$ such that $\theta_n=\arg\min_{\theta\in\Theta}\frac{1}{n}c' \onesmat'\diag(y+f(0)-f(\theta_n))\hspace{1pt}\dmat\hspace{1pt} \diag(y+f(0)-f(\theta_n))\onesmat c$. }
\end{equation}
The $\theta_n$ is optimal in the sense that the implied asymptotic variance $\frac{1}{n}c' \onesmat'\diag\left(y-f(\theta)\right)\hspace{1pt}\dmat\hspace{1pt} \diag\left(y-f(\theta)\right)\onesmat c$ is the smallest when compared with estimators using the same class of parametric models for adjustments.\footnote{If we replace the first-order design matrix $\dmat$ with an identified variance bound $\widetilde{\dmat}$, the implied $\theta_n$ will instead minimize the asymptotic variance bound.} However, it is impossible to construct a sample analog to the criterion above because some entries in $y-f(\theta_n)$ are never observed simultaneously. This is the same problem we encountered in variance estimation, where some pairs of potential outcomes can never be observed simultaneously. 

To identify and estimate $\theta_n$, we can use the first-order conditions as an alternative criterion. If the minimum is achieved in the interior of the parameter space $\Theta$, $\theta_n$ will satisfy the first-order condition:
\begin{equation}
    0=c' \onesmat'\diag(y-f(\theta_n))\hspace{1pt}\dmat\hspace{1pt} \diag\left(\frac{\partial}{\partial \theta_t}f(\theta_n)\right)\onesmat c, t\in [s],
\end{equation}
where $s$ is the number of parameters. Notice that the first order conditions involve only terms with a single potential outcome and hence do no suffer from the the joint-nonobservability problem encountered in (\ref{optimal-gr}).  

Similarly, for a parameter $\theta_t$, we define $\frac{\partial}{\partial \theta_t}f^a(\theta)=\left(\frac{\partial}{\partial \theta_t}f^a(x_1,\theta),...,\frac{\partial}{\partial \theta_t}f^a(x_n,\theta)\right)'\in\mathbb{R}^n$ and the column vector $\frac{\partial}{\partial \theta_t}f(\theta)=\left(\frac{\partial}{\partial \theta_t}f^1(\theta)',\frac{\partial}{\partial \theta_t}f^2(\theta)',...,\frac{\partial}{\partial \theta_t}f^k(\theta)'\right)'\in\mathbb{R}^{kn}$. In other words, $\frac{\partial}{\partial \theta_t}f^a(\theta)$ is the partial derivative of the imputation function with respect to $\theta_t$ evaluated at $\theta$ for all units in arm $a$, and $\frac{\partial}{\partial \theta_t}f(\theta)$ denote the stacked version of such partial derivatives across arms.

A moment estimator for $\theta_n$ is constructed from the population moment vector $g_n(\theta)\in \mathbb{R}^s$. The $t$th entry of the moment vector $g_n(\theta)\in \mathbb{R}^s$ is 
\begin{equation}
    g_{n,t}(\theta)=\frac{1}{n}c'\onesmat'\diag(y-f(\theta))\Ome \diag\left(\frac{\partial}{\partial \theta_t} f(\theta)\right)\onesmat c.   
\end{equation}
Its sample analog $ \widehat{g}_{n,t}(\theta)$ can be expressed as:\footnote{Alternatively, one can use $       \frac{1}{n}c'\onesmat'\diag(y)'\bpiInv\R\Ome \diag(\frac{\partial}{\partial \theta_t} f(\theta))\onesmat c-\frac{1}{n}c'\onesmat'\diag(f(\theta))'\Ome \diag(\frac{\partial}{\partial \theta_t} f(\theta))\onesmat c.$ }
\begin{equation}
 c'\onesmat'\diag(y-f(\theta))'\bpiInv\R\Ome \diag(\frac{\partial}{\partial \theta_t} f(\theta))\onesmat c
\end{equation}
The criterion and its sample analog are 
\begin{equation}\label{M-Optim}
    \mathcal{L}_n(\theta)=g_{n}(\theta)' g_{n}(\theta), \hspace{5pt}  \widehat{\mathcal{L}}_n(\theta)=\widehat{g}_{n}(\theta)'\widehat{g}_{n}(\theta).
\end{equation}
Note that there are $s$ moments for $s$ parameters and hence our model is exactly identified. The Opt-GR estimators are constructed according to Algorithm \ref{Opt-GR}.\\
\begin{algorithm}[h]\label{Opt-GR}
\caption{Opt-GR estimator for $\mu_{n,c}=c'\frac{1}{n}\onesmat'y$ }
\begin{algorithmic}
\Require Parameter space $\Theta$, imputation functions $f^a(\cdot,\theta)$, $a\in[k]$
\begin{enumerate}
\item Define
$\widehat{\mathcal{L}}_n(\theta)=\widehat{g}_{n}(\theta)'\widehat{g}_{n}(\theta)$ as in (\ref{M-Optim}) and obtain $\widehat{\theta}_n\equiv\arg\min_{\theta\in\Theta}\widehat{\mathcal{L}}_n(\theta)$.
    \item  Compute $\widehat{\mu}^{\toc}_{n,a}$, for $a=1,...,k$, where
    \begin{equation*}\
        \widehat{\mu}_{n,a}^{\toc} = \frac{1}{n}\sum_{i=1}^n f^a(x_i,\widehat{\theta}_{n}) + \frac{1}{n}\sum_{i=1}^n\frac{\R_{ai}}{\bpi_{ai}}  (y_{ai}-f^a(x_i,\widehat{\theta}_{n})).
    \end{equation*}
    \item Output $\widehat{\mu}_{n,c}^{\toc}=\sum_{a=1}^k c_a\widehat{\mu}^{\toc}_{n,a}$. 
\end{enumerate}
\end{algorithmic}
\end{algorithm}
Theoretical guarantees can be derived with the following identification assumptions, with additional standard regularity assumptions (Assumption \ref{A:GMM2}) wich we include in Appendix \ref{regularity_assumptions}.
\begin{assumption}\label{A:GMM1} There exists a positive integer $N$ such that for all $n\geq N$ the following conditions hold:
\begin{enumerate}[label=(\roman*)] 
    \item The parameter space $\Theta$ is a compact set in $\mathbb{R}^{s}$ with a nonempty interior. 
    \item There exists a $\theta_n$ and a positive $c_{\ref{A:GMM1},1}$ such that, for any $\epsilon>0$, $\inf_{\theta\in \Theta\backslash B(\theta_n,\epsilon)}\mathcal{L}_n(\theta)-\mathcal{L}_n(\theta_n)>c_{\ref{A:GMM1},1}\epsilon^2$. Moreoever, there exists a $\delta$ such that $\text{dist}(\theta_n,\mathrm{Bd}(\Theta))>\delta$.
\end{enumerate}
\end{assumption}

Define $\widehat{\mu}_{n,a}^{\toc,\tL}$, $\widehat{\mu}_{n,c}^{\toc,\tL}=\sum_{a=1}^k c_a\widehat{\mu}_{n,a}^{\toc,\tL}$, and $ \V(\widehat{\mu}_{n,c}^{\toc,\tL})$ as in (\ref{qmle_linearized}) and (\ref{qmle_variance}), but with $\theta_n$ replaced by $\theta_n\equiv\arg\min_{\theta\in\Theta} \mathcal{L}_n(\theta)$ where $\mathcal{L}_n(\theta)$ is defined in (\ref{M-Optim}).
\begin{theorem}\label{Thm:OC}
Define $\widehat{\theta}_n$,  $\widehat{\nu}_{n,a}^{\toc}$, and $\widehat{\mu}_{n,c}^{\toc}$ as in Algorithm \ref{Opt-GR}.Under Assumptions \ref{A:BoundedFourthMoments},\ref{A:GMM1}, and \ref{A:GMM2} and if $\viiii{\dmat}_1=O(1)$, $\sigma_{\max}((\widetilde{\dmat}\otimes \widetilde{\dmat})\circ \s)=o(n)$, and
$\sigma_{\max}\left(\dtildep\right)=O(1)$, and there exists a positive constant $c_{\ref{Thm:OC}}$ such that $n\V(\widehat{\mu}_{n,c}^{\toc,\tL})\geq c_{\ref{Thm:OC}}$ uniformly for all large $n$, then following results hold: \\
\begin{enumerate}[label=(\roman*)]
   \item We have $\left(\widehat{\mu}^{\toc}_{n,c}-\widehat{\mu}_{n,c}^{\toc,\tL}\right)/\sqrt{\V(\widehat{\mu}_{n,c}^{\toc,\tL})}=o_p\left(1\right)$. 
   \item $ \V(\widehat{\mu}_{n,c}^{\toc,\tL})= \min_{\theta\in\Theta}\frac{1}{n}c' \onesmat'\diag\left(y-f(\theta)\right)\hspace{1pt}\dmat\hspace{1pt} \diag\left(y-f(\theta)\right)\onesmat c$
\item Define the variance bound $\widetilde{\V}(\widehat{\mu}_{n,c}^{\toc,\tL})$  as in (\ref{qmle_vbound}),with an identified variance bound matrix $\widetilde{\dmat}$,  and the the plug-in variance-bound estimator $\widehat{\widetilde{\V}}(\widehat{\mu}_{n,c}^{\toc,\tL})$ as in (\ref{qmle_vbound_est}). The variance bound estmiator is consistent
is consistent: $\widehat{\widetilde{\V}}(\widehat{\mu}_{n,c}^{\toc,\tL})/\widetilde{\V}(\widehat{\mu}_{n,c}^{\toc,\tL})\overset{p}{\to} 1$. 
\item If there exists $q_{\alpha}$ such that $\lim_{n\to\infty}\textrm{P}_n\left(\left|\widehat{\mu}_{n,c}^{\toc,\tL}-\mu_{n,c}\right|\geq q_{\alpha}\sqrt{\V(\widehat{\mu}_{n,c}^{\toc,\tL})}\right)\leq \alpha$,
then, $\lim_{n\to\infty}\textrm{P}_n\left(\left|\widehat{\mu}_{n,c}^{\toc}-\mu_{n,c}\right|\geq q_{\alpha}\sqrt{  \widehat{\widetilde{\V}}(\widehat{\mu}_{n,c}^{\toc,\tL})}\right)\leq \alpha $. 
\end{enumerate}
\end{theorem} 
\begin{remark}
\textcolor{red}{
Our notion of optimality in Theorem \ref{Thm:OC}-(ii) and (\ref{optimal-gr}) is weaker than the semiparametric efficiency bound commonly used in the i.i.d. sampling literature \cite{bickel1993efficient}. To our knowledge, this notion of semiparametric efficiency has not been developed in the design-based statistical literature. Instead, our definition of estimator optimality aligns with that of \cite{lin2013agnostic} and \cite{middleton2018unified}: we consider an estimator optimal if it achieves the smallest asymptotic variance, within a given class of adjustments.}
\end{remark}
\begin{remark}
We now comment on Assumption \ref{A:GMM1}-(ii) extensively. Identifiability is a very important assumption here. In general, there can be multiple optimal solutions depending on the adjustment strategy (\cite{lin2013agnostic,middleton2018unified}). This is because some experimental designs will make the GR estimator invariant to certain parameter choices. For example, consider the setting of a two-arm  completely randomized design with one pretreatment covariate. Let 1 denote the treatment arm and 0 denote the control arm, and let $n_1$ and $n_0$ denote the number of treated and control units, respectively. Define $\Bar{x}=\frac{1}{n}\sum_{i}x_i=0$ (centered), $\widehat{\Bar{x}}_1 =\frac{1}{n_1}\sum_{i}\R_{1i}x_i$, and $\widehat{\Bar{x}}_0 =\frac{1}{n_0}\sum_{i}\R_{0i}x_i$, and note $\widehat{\Bar{x}}_0=-\frac{n_1}{n_0}\widehat{\Bar{x}}_1$. Suppose we use a separate-slope linear model to adjust $f^0(x_i,\beta)=\beta_0+\beta_1 x_i$ and $f^1(x_i,\beta)=\beta_2+\beta_3 x_i$ and $\frac{1}{n}\sum_{i=1}^n x_i=0$. The GR estimator for the ATE is
\begin{align}
   & (\beta_2-\beta_0)+\frac{1}{n}\sum_{i}x_i(\beta_3-\beta_1)-\left(\frac{1}{n_1}\sum_{i}\R_{1i}(\beta_2+x_i\beta_3)-\frac{1}{n_0}\sum_{i}\R_{0i}(\beta_0+x_i\beta_1)\right)\\
    & =0 - \widehat{\Bar{x}}_1\beta_3 +  \widehat{\Bar{x}}_0\beta_1 = -\widehat{\Bar{x}}_1\left(\beta_3 + \frac{n_1}{n_0}\beta_1\right).        
\end{align}
We observe that the intercepts $\beta_0$ and $\beta_2$ are canceled and that there are multiple pairs of $(\widetilde{\beta}_1,\widetilde{\beta}_3)$ that are equivalent to $(\beta_1,\beta_3)$, such as $\widetilde{\beta}_1=0$ and $\widetilde{\beta}_3=\beta_3 + \frac{n_1}{n_0}\beta_1$.\footnote{We note that the identification problem highlighted here is design specific. For example, this problem will also arise for pairwise randomized designs but not for Bernoulli designs.} 

In general, there are two sources of the weak/non-identification problem. The first is weak/non identification of arm-specific intercepts. This typically happens when the number of units in an arm is fixed in all possible random treatment allocations. Another source of weak/non identification is that the design induces co-linearity and  cancellation of covariates coefficients.

For linear models, both problems can be detected by inspecting the eigenvalues of $\frac{1}n{}\X\dmat\X$. Small eigenvalues correspond to the possible cancellation of covariate coefficients or arm-specific intercepts. To use the Opt-GR estimators, we recommend that researchers inspect these eigenvalues of before applying the estimators. If one of the eigenvalues is small, the researcher may wish, for example, to avoid specifying an intercept for the treatment arms or use a model with same-slope adjustments instead of a model with separate-slope adjustments. 
    
\end{remark}


We end this section by noting that one can combine the insights of No-harm GR and Opt-GR estimators to form a class of Optimal-Imputed (Opt-I) GR estimators. This class of estimators is Opt-GR estimators with a linear imputation function. Instead of using the full set of covariates, the linear imputation function uses a single covariate imputed by a QMLE model (for example, a flexible ML model).\footnote{We note that the coefficient estimator for the optimal-GR estimator with linear imputation functions admits a closed-form solution.} We find that this class of estimators has good finite-sample performance in our simulations. We detail the constructions below. Recall the definition of the intercept matrix $\onesmat$ in equation (\ref{intercept}) and the stack of imputations $f(\theta)$ defined before Section \ref{Section:Nonlinear}. The assumptions, asymptotic theory, and variance-bound estimation are left to Appendix \ref{more_results_S5} due to space constraints.
\begin{algorithm}[h]\label{OCI-GR}
\caption{Opt-I estimator for $\mu_{n,c}=c'\frac{1}{n}\onesmat'y$ }
\begin{algorithmic}
\Require QMLE coefficient estimates $\widehat{\theta}_n$ from Algorithm \ref{QMLE-GR}, imputation functions $f^a(\cdot,\theta)$, $a\in[k]$
\begin{enumerate}
    \item Define $\widehat{X}=\begin{bmatrix}
        \onesmat &\vert f(\widehat{\theta}_n)
    \end{bmatrix}\in \mathbb{R}^{kn\times(k+1)}$.
    \item Define $\widehat{g}_n(\beta)= \allowdisplaybreaks \widehat{X}'\diag(c'\onesmat)\dmat\diag(c'\onesmat)\R\bpiInv\left(y-\widehat{X}\beta\right)\in \mathbb{R}^{(k+1)\times 1}$.
    \item Define $\widehat{\beta}=[\widehat{\beta}^1,...,\widehat{\beta}^{k+1}]=\min_{\beta}\left(\widehat{g}_n(\beta)'\widehat{g}_n(\beta)\right)$.
    \item  Compute $\widehat{\mu}_{n,a}^{\toci}$, for $a\in [k]$, where
    {\small
    \begin{equation}\label{DR}
        \widehat{\mu}_{n,a}^{\toci} = \frac{1}{n}\sum_{i=1}^n \left(\widehat{\beta}^a + \widehat{\beta}^{k+1}f^a(x_i,\widehat{\theta}_n)\right) + \frac{1}{n}\sum_{i=1}^n\frac{\R_{ai}}{\bpi_{ai}}  \left(y_{ai}-\widehat{\beta}^a - \widehat{\beta}^{k+1}f^a(x_i,\widehat{\theta}_n)\right).
    \end{equation}}
    \item Output $\widehat{\mu}_{n,c}^{\toci}=\sum_{a=1}^k c_a\widehat{\mu}_{n,a}^{\toci}$. 
\end{enumerate}
\end{algorithmic}
\end{algorithm}


\begin{comment}
\subsubsection{Weighted Nonlinear Least Squares}\label{WNLS}
\hspace{20pt}\\ \indent We first define the column vector
$f^a(\theta)=\left[f^a(x_1,\theta),...,f^a(x_n,\theta)\right]\in\mathbb{R}^n$, and the column vector $f(\theta)=\left[f^1(\theta)',f^2(\theta)',...,f^k(\theta)'\right]'\in\mathbb{R}^{kn}$.  In words, $f^a(\theta)$ is the imputed potential outcomes for all units in arm $a$ with parameter $\theta$. $f(\theta)$ is the stack of the imputed outcomes of all arms. \\
\indent For the weighted nonlinear least squares, the $M$-criterion and its sample equivalent are:
\begin{itemize}
    \item $\mathcal{L}_n(\theta)=-\frac{1}{n}c'\onesmat'\diag(y-f(\theta))'\widetilde{\Ome}\diag(y-f(\theta))\onesmat c$
    \item $ \widehat{\mathcal{L}}^2_n(\theta)=-\frac{1}{n}c'\onesmat'\diag(y-f(\theta))'\R\Otildep \R\diag(y-f(\theta))\onesmat c	\\\text{\hspace{9.5mm}}=-\frac{1}{n}c'\onesmat'\R\diag(y-f(\theta))'\R\Otildep \R\diag(y-f(\theta))\R\onesmat c$
\end{itemize}
$\widetilde{\Ome}\in \mathbb{R}^{kn\times kn}$ is a positive definite matrix, and $\Otildep: = \widetilde{ \Ome } / \matp$
where $\matp$ is defined in Definition \ref{SO} and $/$ denotes element-wise division defined such that division by zero equals zero. Note here we are implicitly assuming the pointwise division in $\Otildep$ is well-defined: entries in $\Ome$ have to be zero when the corresponding entries in $\matp$ are zero. The motivating example here is $\widetilde{\Ome}=\widetilde{\mathbf{D}}$, where $\widetilde{\mathbf{D}}$ is a valid variance bounding matrix.  
\begin{assumption}\label{A1-WNLS} The following conditions are satisfied:
\begin{enumerate}
    \item (Parameter Space) Let $s$ be a positive integer. The parameter space $\Theta$ is a compact set in $\mathbb{R}^{s}$ with nonempty interior. Let $d(\cdot,\cdot)$ denote a metric on $\Theta$.
    \item (Interior Solution) There exists a $\theta_n$ such that, for any $\epsilon>0$, $\inf_{\theta\in \Theta\backslash B(\theta_n,\epsilon)}\mathcal{L}_n(\theta)>\mathcal{L}_n(\theta_n)$. Moreoever, $\text{dist}(\theta_n,\text{Bd}(\Theta))>\epsilon$ uniformly in $n$.
    \item (First Order Expansion) $|f^a(x_i,\theta_2)-f^a(x_i,\theta_1)|\leq D^{a}_{\ref{A1-WNLS}}(x_i)h(d(\theta_1,\theta_2))$ for all $\theta_1,\theta_2\in\Theta$. $h$ is a function that does not change with $n$ and satisfies $h(t)\to 0 $ as $t\to 0$. $D^a(\cdot)$ is a non-negative function of $x_{i}$. There exists a $C_{\ref{A1-WNLS},5}$ such that $\frac{1}{n}\sum_{a,i} (D^{a}_{\ref{A1-WNLS},1}(x_i))^2<C_{\ref{A1-WNLS},5}$ for all $n$.
    \item (Moments 1) For all $\theta\in\Theta$, there exists a $C_{\ref{A1-WNLS},3}$ such that $\frac{1}{n}\sum_{a,i} \left[ y_{ai}-f^a(x_i,\theta)\right]^4<C_{\ref{A1-WNLS},3}$  for all $n$.
    \item (Moments 2) At $\theta_n$ and for all $n$, there exists a $C_{\ref{A1-WNLS},7}$ such that $\frac{1}{n}\sum_{a,i}\left(\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)\right)^4\leq C_{\ref{A1-WNLS},7}$ and $C_{\ref{A1-WNLS},7}$ such that $\frac{1}{n}\sum_{a,i}\left(\frac{\partial^2}{\partial \theta_t\partial \theta_u}f^a(x_i,\theta)\right)^4\leq C_{\ref{A1-WNLS},7}$ for all $k,u=1,...,s$
    \item (First Order Expansion for First Derivatives) $|\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)- \frac{\partial}{\partial \theta_t}f^a(x_i,\theta_n)|\leq D^{a}_{\ref{A1-WNLS},2}(x_i) ||\theta-\theta_n||_2$ for all $k=1,...,s$. There exists a $C_{\ref{A1-WNLS},8}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A1-WNLS},2}(x_i))^2 \leq C_{\ref{A1-WNLS},8}$ for all $n$.
    \item (Second Order Expansion)$|f^a(x_i,\theta)- f^a(x_i,\theta_n)-\nabla_{\theta}f^a(x_i,\theta_n)'(\theta-\theta_n)|\leq D^{a}_{\ref{A1-WNLS},3}(x_i) ||\theta-\theta_n||^2_2$ for all $t=1,...,s$.   $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A1-WNLS},3}(x_i))^2 \leq C_{\ref{A1-WNLS},8}$
    \item (Second Order Expansion for First derivatives) $|\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)- \frac{\partial}{\partial \theta_t}f^a(x_i,\theta_n)-\nabla_{\theta_k\theta}f^a(x_i,\theta_n)'(\theta-\theta_n)|\leq D^{a}_{\ref{A1-WNLS},4}(x_i) ||\theta-\theta_n||^2_2$ for all $t=1,...,s$. There exists a $C_{\ref{A1-WNLS},8}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A1-WNLS},4}(x_i))^2 \leq C_{\ref{A1-WNLS},9}$.
    \item (Designs) $\sigma_{\max}((\widetilde{\Ome}\otimes \widetilde{\Ome})\circ \s)=o(n)$, $|||\Otildep|||=O_p(1)$
    \item (Local Identification) The smallest absolute eigenvalue of  $\frac{1}{n}\sum_{ai}\sum_{a'i'}\widetilde{\Ome}_{aia'i'}\nabla f^a(x_i,\theta_n)\nabla f(x_{i'},\theta_n)' -\frac{1}{n}\sum_{ai}\sum_{a'i'}\widetilde{\Ome}_{aia'i'}(y_{ai}-f^a(x_i,\theta_n))\nabla_{\theta\theta} f(x_{i'},\theta_n)$ is bounded away from 0 for all $n\geq N$.
\end{enumerate}
\begin{theorem}
Under Assumption 13, $\widehat{\theta}_n-\theta_n=O(\sqrt{\frac{1}{n}\sigma_{\max}((\widetilde{\Ome}\otimes \widetilde{\Ome})\circ \s)})$
\end{theorem}
\end{assumption}

\begin{assumption}\label{A:GMM2} Let $\theta_n$ be defined in Assumption \ref{A:GMM1}. Let $N$ be a positive integer.  Uniformly for all $n\geq N$, the following conditions are satisfied:
\begin{enumerate}[label=(\roman*)] 
\item (Moments)
\begin{enumerate}
   \item (Criterion Moments) For all $\theta\in\Theta$, there exists a $C_{\ref{A:GMM2},1}$ such that $\frac{1}{n}\sum_{a,i} \left( y_{ai}-f^a(x_i,\theta)\right)^4<C_{\ref{A:GMM2},1}$.
    \item (Derivative Moments) For all $\theta\in\Theta$,  there exists a $C_{\ref{A:GMM2},2}$ such that $\frac{1}{n}\sum_{a,i}\left(\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)\right)^4\leq C_{\ref{A:GMM2},2}$ and  $\frac{1}{n}\sum_{a,i}\left(\frac{\partial^2}{\partial \theta_t\partial \theta_u}f^a(x_i,\theta)\right)^4\leq C_{\ref{A:GMM2},2}$ for all $t,u\in [s]$.
\end{enumerate}
    \item  (Lipschitz Continuity for the Function and Its Derivatives) For all $a\in [k]$.
\begin{enumerate}
    \item  $f^a(x_i,\theta)$ is two-times differentiable in $\theta$ for all $x_i$, $i\in [n]$.
    \item  (Function) For all $\theta_1,\theta_2\in\Theta$, $|f^a(x_i,\theta_2)-f^a(x_i,\theta_1)|\leq D^{a}_{\ref{A:GMM2},3}(x_i)\|\theta_2-\theta_1\|_2$. There exists a $C_{\ref{A:GMM2},3}$ such that $\frac{1}{n}\sum_{a,i} (D^{a}_{\ref{A:GMM2},3}(x_i))^2<C_{\ref{A:GMM2},3}$.
     \item (First Derivatives)  For all $\theta_1,\theta_2\in\Theta$, $|\frac{\partial}{\partial \theta_t}f^a(x_i,\theta_2)- \frac{\partial}{\partial \theta_t}f^a(x_i,\theta_1)|\leq D^{a}_{\ref{A:GMM2},4}(x_i) \|\theta_2-\theta_1\|_2$ for all $k\in [s]$. There exists a $C_{\ref{A:GMM2},4}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},4}(x_i))^2 \leq C_{\ref{A:GMM2},4}$. 
     \item (Second Derivatives) There exists a $\epsilon$ such that for all $\theta\in B(\theta_n,\epsilon)$,  $|\frac{\partial^2}{\partial \theta_t\partial \theta_u}f^a(x_i,\theta)- \frac{\partial^2}{\partial \theta_t\partial \theta_u}f^a(x_i,\theta_n)|\leq D^{a}_{\ref{A:GMM2},5}(x_i) \|\theta-\theta_n\|_2$ for all $t,u\in [s]$. There exists a $C_{\ref{A:GMM2},5}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},5}(x_i))^2 \leq C_{\ref{A:GMM2},5}$. 
\end{enumerate}    
    \item (Taylor Approximations) For all $a\in [k]$,
\begin{enumerate}
    \item (First-Order Approximation for the Function) There exists an $\epsilon$ such that for all $\theta\in B(\theta_n,\epsilon)$,,  $|f^a(x_i,\theta)- f^a(x_i,\theta_n)-\nabla_{\theta}f^a(x_i,\theta_n)'(\theta-\theta_n)|\leq D^{a}_{\ref{A:GMM2},6}(x_i) \|\theta-\theta_n\|^2_2$ for all $t\in [s]$.   $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},6}(x_i))^2 \leq C_{\ref{A:GMM2},6}$.
    \item (First-Order Approximation for the First Derivative) There exists an $\epsilon$ such that for all $\theta\in B(\theta_n,\epsilon)$,  $|\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)- \frac{\partial}{\partial \theta_t}f^a(x_i,\theta_n)-\nabla_{\theta} (\frac{\partial}{\partial \theta_t}f^a(x_i,\theta_n))'(\theta-\theta_n)|\leq D^{a}_{\ref{A:GMM2},7}(x_i) \|\theta-\theta_n\|^2_2$ for all $t\in [s]$. There exists a $C_{\ref{A:GMM2},7}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},7}(x_i))^2 \leq C_{\ref{A:GMM2},7}$.
\end{enumerate}
\item There exists a positive scalar $\epsilon$ such that the smallest absolute eigenvalue of the matrix \\$d g_n(\theta_n)\in \mathbb{R}^{s\times s}$  is greater than $\epsilon$, where $d g_n(\theta_n)$ is the differential of $g_n$ evaluated at $\theta_n$.   
\end{enumerate}
\end{assumption}
\begin{remark}
Assumption \ref{A:GMM2} can be checked by a Taylor expansion of the imputation functions coupled with appropriate moment conditions. 
\begin{comment}
2) Always inspect the eigenvalues of $\X'\Ome\X$; if the eigenvalues are very close to zero, try removing some covariate columns;  3) One could add some penalty terms onto the criterion, for example $\mathcal{L}_n(\theta)+\|\theta\|^2_2$. Solution to this problem is no longer optimal. However, one may gain identification and improved finite-sample performance in exchange for a loss of efficiency.
\end{comment}
\end{remark}




%%%%%%OLD PROOFS FOR OPTIMAL GR ESTIMATOR%%%%%%%

\subsection{Proof of Theorem \ref{Thm:OC}}
Notice first:
\begin{itemize}
    \item $\left(1-\pi_{ai}\right)/\pi_{ai}\leq \sigma_{\max}\left(\dmat\right)$ for all $a\in[k]$ and $i\in[n]$ because $\dmat$ is positive-semidefinite and $\V\left(\R_{ai}/\pi_{ai}\right)=\left(1-\pi_{ai}\right)/\pi_{ai}$ is on the diagonal of $\dmat$. This implies $\max_{a,i}\{1/\pi_{ai}\}\leq \sigma_{\max}\left(\dmat\right)+1$. 
    \item $\sigma_{\max}\left(\dmat\right)\leq\viiii{\dmat}_1$ by Lemma 5.6.10 in \cite{horn2012matrix}.
\end{itemize}
We only need to check the $\sqrt{n}$-consistency $\hat{\theta}_n$. The rest proofs are identical to those of Theorem \ref{Thm:QMLE}.
We first check the pointwise convergence of the criterion, namely
\begin{equation*}
    \widehat{\mathcal{L}}_n(\theta)- \mathcal{L}_n(\theta)=o_p(1),
\end{equation*}
pointwise in $\theta\in\Theta$. For this we show,
\begin{equation*}
  \widehat{g}_n(\theta)- g_n(\theta)=o_p(1).
\end{equation*}
First note that $\widehat{g}_n(\theta)$ is an unbiased estimator of $g_n(\theta)$. We adopt the notation $y^c$ and $f^c\left(\theta\right)$ in the proof of Theorem \ref{Thm:NOHARM}. In addition, we define $\frac{\partial}{\partial \theta_t}f^c(\theta)\equiv c'\onesmat'\diag(\frac{\partial}{\partial \theta_t} f(\theta))\in \mathbb{R}^{kn}$.  Let $\nabla_{\theta} f^c(\theta)\in \mathbb{R}^{kn\times s}$ denote the column stacks of $\frac{\partial}{\partial \theta_t}f^c(\theta), t\in [s]$ .\\
The variance of $g_n(\theta)$ is $n^{-1}\left(y^c-f^c(\theta)\right)\bpiInv\R\Ome \frac{\partial}{\partial \theta_t}f^c(\theta)$ is:
\begin{align*}
    &\frac{1}{n^2}\V\left(\left(y^c-f^c(\theta)\right)\bpiInv\R\Ome\frac{\partial}{\partial \theta_t}f^c(\theta)\right)\\
    =& \frac{1}{n^2} \V\left(1_{\scriptscriptstyle kn}'\diag\left(y^c-f^c(\theta)\right)\bpiInv\R\Ome\frac{\partial}{\partial \theta_t} f^c(\theta)\right)\\
    = &   \frac{1}{n^2} \V\left(1_{\scriptscriptstyle kn}'\bpiInv\R\diag(y^c-f^c(\theta))\Ome\frac{\partial}{\partial \theta_t} f^c(\theta)\right)\\
     =&  \frac{1}{n^2}\frac{\partial}{\partial \theta_t} f^c(\theta)'\Ome'\diag\left(y^c-f^c(\theta)\right)\dmat \diag\left(y^c-f^c(\theta)\right)\Ome \frac{\partial}{\partial \theta_t} f^c(\theta)\\
    \leq &   \sigma_{\max}\left(\dmat\right) \times \left(\frac{1}{n^2}\frac{\partial}{\partial \theta_t} f^c(\theta)'\Ome'\diag\left(y^c-f^c(\theta)\right)\diag\left(y^c-f^c(\theta\right)\Ome \frac{\partial}{\partial \theta_t} f^c(\theta)\right)\\
     \leq &  \frac{\viiii{\Ome}_1^2\sigma_{\max}\left(\dmat\right)}{n} \sqrt{\frac{1}{n}\sum_{a,i} \left(c_a y_{i}(a)-c_a f(x_i,\theta)\right)^4}\times  \sqrt{\frac{1}{n}\sum_{a,i} (c^a\frac{\partial}{\partial \theta_t} f^a(x_i,\theta))^4}
\end{align*}
where for the last inequality we use Lemma \ref{Lemma:bound}. Under A\ref{A:GMM1}-(i) and A\ref{A:GMM2}, the term above is $o_p(1)$. Since $g_n(\theta)$ is $O(1)$ by A\ref{A:GMM2}-(i), we have $\widehat{g}_n(\theta)'\widehat{g}_n(\theta)-g_n(\theta)g_n(\theta)=o_p(1)$ pointwise in $\theta$. \\
Next we check stochastic equicontinuity as in the proof of Theorem \ref{Thm:QMLE}. First, the $t$th entry of $\widehat{g}_n(\theta)$ can be upper bounded by
\begin{align*}
 &\frac{1}{n}\left(y^c-f^c(\theta)\right)'\bpiInv\R\dmat\frac{\partial}{\partial \theta_t} f^c(\theta) \\
 \leq & \sigma_{\max}\left(\dmat\right) \times \max_{a,i}\{\frac{1}{\pi_{ai}}\}\sqrt{\frac{1}{n}\sum_{a,i}(c_a y_{i}(a)-c_a f(x_i,\theta))^2}  \sqrt{\frac{1}{n}\sum_{a,i}\left(c_a\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)\right)^2} \\
 \leq & C,
\end{align*}
for a $C$ bounded above uniformly for large $n$ by Assumption \ref{A:GMM2}-(i).
Then we bound:
\begin{align}
    &\hat{g}_n(\theta_1)'\hat{g}_n(\theta_1) -  \hat{g}_n(\theta_2)'\hat{g}_n(\theta_2) \\
    =& (\hat{g}_n(\theta_1)-\hat{g}_n(\theta_2))'\hat{g}_n(\theta_1)-  \hat{g}_n(\theta_2)'(\hat{g}_n(\theta_1)-\hat{g}_n(\theta_2))\\
    \leq &  \|\hat{g}_n(\theta_1)\|_2 \times \|\hat{g}_n(\theta_1)-\hat{g}_n(\theta_2)\|_2 +  \|\hat{g}_n(\theta_2)\|_2 \times \|\hat{g}_n(\theta_1)-\hat{g}_n(\theta_2)\|_2\\
    \leq &2C\times \|\hat{g}_n(\theta_1)-\hat{g}_n(\theta_2)\|_2,
\end{align}
We have for the $t$th entry of $\hat{g}_n(\theta_1)-\hat{g}_n(\theta_2)$
\begin{align}
   &\frac{1}{n}\left(y^c-f^c(\theta_1)\right)'\bpiInv\R\Ome \left(\frac{\partial}{\partial \theta_t} f^c(\theta_1)-\frac{\partial}{\partial \theta_t} f^c(\theta_2)\right)\\
   +& \frac{1}{n}(f^c(\theta_2)-f^c(\theta_1))'\bpiInv\R\Ome\frac{\partial}{\partial \theta_t}f^c(\theta_2)\\
    \leq & \sigma_{\max}\left(\dmat\right)\times \max_{a,i}\{\frac{1}{\pi_{ai}}\} \times \\
    & \sqrt{\frac{1}{n}\sum_{a,i}(c_a y_{i}(a)-c_af^a(x_i,\theta_1))^2} \sqrt{\frac{1}{n}\sum_{a,i}(c_a\frac{\partial}{\partial t}f^a(x_i,\theta_1)-c_a\frac{\partial}{\partial t}f^a(x_i,\theta_2))^2} \\  
    +&  \sigma_{\max}\left(\dmat\right)\times \max_{a,i}\{\frac{1}{\pi_{ai}}\} \times\sqrt{\frac{1}{n}\sum_{a,i}(c_af^a(x_i,\theta_1)-c_af^a(x_i,\theta_2))^2} \times\\
    & \sqrt{\frac{1}{n}\sum_{a,i}(c_a\frac{\partial}{\partial \theta_t}f^a(x_i,\theta_1))^2}\\
    \leq &   C\|\theta_1-\theta_2\|_2,  \label{(26)}  
\end{align}
for a $C$ bounded above uniformly for large $n$. 
The last line is justified by Assumptions \ref{A:GMM2}-(i), \ref{A:GMM2}-(ii)-(b), \ref{A:GMM2}-(ii)-(c) and $\sigma_{\max}(\Ome)$. Using the same steps as in Theorem \ref{Thm:QMLE}, we can prove stochastic equicontinuity upon noticing
\begin{align}
    & \mathbf{P}_n(|\hat{g}_n(\theta_1)'\hat{g}_n(\theta_1)-\hat{g}_n(\theta_2)'\hat{g}_n(\theta_2)|>2\epsilon)\\
      \leq & \mathbf{P}_n(\|\hat{g}_n(\theta_2)-\hat{g}_n(\theta_1)\|_2\times \|\widehat{g}_n(\theta_1)\|_2>\epsilon ) \\
      & +\mathbf{P}_n(\|\hat{g}_n(\theta_2)-\hat{g}_n(\theta_1)\|_2\times \|\hat{g}_n(\theta_2)\|_2>\epsilon )\\
    \leq & \mathbf{P}_n(C\|\theta_2-\theta_1\|_2\times \|\hat{g}_n(\theta_1)\|_2>\epsilon )\\
    & +\mathbf{P}_n(C\|\theta_2-\theta_1\|_2\times \|\hat{g}_n(\theta_2)\|_2>\epsilon )\to 0 
\end{align}
as $\|\theta_1-\theta_2\|_2\to 0$, where we use the fact that $\widehat{g}_n(\theta)$ is uniformly bounded above by a constant $C$. Further with Assumption \ref{A:GMM1}-(ii) and by Lemma \ref{Lemma:SC} and \ref{Lemma:UC}, we have $\hat{\theta}_n-\theta_n=o_p(1)$.\\
tablish the rate of convergence. By Assumption \ref{A:GMM1}-(ii), with probably approaching one, $\hat{\theta}_n$ is in the interior of $\Theta$ and satisfies the first order condition. We have:
\begin{equation}\label{eq:25}
    \hat{g}_n(\hat{\theta}_n)'\nabla_{\theta}\hat{g}_n(\hat{\theta}_n)=\0 \in \mathbb{R}^{s\times 1}
\end{equation}
For the $t$th entry of the equalities above, it can be written as:
\begin{equation*}
    \sum_{r=1}^s\hat{g}_{n,r}(\hat{\theta}_n)\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\hat{\theta}_n)=0.
\end{equation*}
We expand:
\begin{align*}
    0 = & \sum_{r=1}^s \hat{g}_{n,r}\left(\theta_n\right)\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}\left(\theta_n\right) +  \underbrace{\sum_{r=1}^s \left(\hat{g}_{n,r}\left(\hat{\theta}_n\right)-\hat{g}_{n,r}(\theta_n)\right)\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}\left(\theta_n\right)}_{(A)}\\
    &+ \underbrace{\sum_{r=1}^s \hat{g}_{n,r}\left(\theta_n\right)\left(\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\hat{\theta}_n)-\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)\right)}_{(B)}\\
    & + \underbrace{\sum_{r=1}^s 
    \left(\hat{g}_{n,r}(\hat{\theta}_n)-\hat{g}_{n,r}(\theta_n)\right)\left(\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\hat{\theta}_n)-\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)\right)}_{(C)}
\end{align*}
To study (A), (B) and (C), we study the terms $\hat{g}_{n,r}(\hat{\theta}_n)-\hat{g}_{n,r}(\theta_n)$ and $\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\hat{\theta}_n)-\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)$. We have as (\ref{(26)}) that $ |\hat{g}_{n,r}(\hat{\theta}_n)-\hat{g}_{n,r}(\theta_n)=O\left(\|\hat{\theta}_n-\theta_n\|_2\right)$. We now study $\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\hat{\theta}_n)-\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)$. Note,
\begin{align}
    \frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta) = -\frac{\partial}{\partial \theta_t}f^c(\theta)\bpiInv\R\Ome\frac{\partial}{\partial \theta_r}f^c(\theta) + \left(y^c-f^c(\theta)\right)\Ome\frac{\partial^2}{\partial \theta_t\theta_r}f^c(\theta) 
\end{align}
We have: 
\begin{align}
    &\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}\left(\hat{\theta}_n\right)-\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}\left(\theta_n\right)\\
     =&  -\frac{\partial}{\partial \theta_t}f^c\left(\hat{\theta}_n\right)\bpiInv\R\Ome\frac{\partial}{\partial \theta_r}f^c\left(\hat{\theta}_n\right) + \left(y^c-f^c\left(\hat{\theta}_n\right)\right)\Ome\frac{\partial^2}{\partial \theta_t\theta_r}f^c\left(\hat{\theta}_n\right) \\
     &-\left(-\frac{\partial}{\partial \theta_t}f^c
    \left(\theta_n\right)'\Ome\frac{\partial}{\partial \theta_r}f^c
    \left(\theta_n\right) + \left(y^c-f^c\left(\theta_n\right)\right)\Ome\frac{\partial^2}{\partial \theta_t\theta_r}f^c\left(\theta_n\right) \right)\\
    = & O(\|\hat{\theta}_n-\theta_n\|_2),
\end{align}
by Assumptions \ref{A:GMM2}-(i), (ii), the fact that $\viiii{\dmat}_1=O(1)$, and using a similar argument as in (\ref{(26)}). Note $\nabla_{\theta}f^c(\theta_n)\in\mathbb{R}^{kn\times s}$ and $\nabla_{\theta}\frac{\partial}{\partial \theta_r}f^c(\theta_n)\in\mathbb{R}^{kn\times s}$ is a matrix of the stacked partial derivatives of $f^c(x_i,\theta_n)$ and $\frac{\partial}{\partial \theta_r}f^c(x_i,\theta_n)$ with respect to $\theta$. Let $\theta_{n,t}$ denote the $t$th element of $\theta_n$ and $\hat{\theta}_{n,t}$ denote the $t$th element of $\hat{\theta}_n$, a Taylor expansion argument gives:
\begin{align*}
    & \hat{g}_{n,r}(\hat{\theta}_n)-\hat{g}_{n,r}(\theta_n)\\
    =  &\left(f^c(\theta_n)-f^c(\hat{\theta}_n)\right)'\bpiInv\R\Ome \frac{\partial}{\partial \theta_r} f^c(\theta_n)\\
    & + \left(y^c-f^c\left(\theta_n\right)\right)'\bpiInv\R\Ome \left( \frac{\partial}{\partial \theta_r} f^c(\hat{\theta}_n)-  \frac{\partial}{\partial \theta_r}f^c(\theta_n)\right)\\
    &+\left(f^c(\theta_n)-f^c(\hat{\theta}_n)\right)'\bpiInv\R\Ome \left( \frac{\partial}{\partial \theta_r} f^c(\hat{\theta}_n)-  \frac{\partial}{\partial \theta_r}f^c(\theta_n)\right)\\
    = & -\left(\nabla_{\theta} f^c(\theta_n)(\hat{\theta}_n-\theta_n)\right)'\bpiInv\R\Ome \frac{\partial}{\partial \theta_r} f^c(\theta_n)\\
    & + \left(f^c(\hat{\theta}_n)-f^c(\theta_n) -\nabla_{\theta} f^c(\theta_n)(\hat{\theta}_n-\theta_n)\right)'\bpiInv\R\Ome \frac{\partial}{\partial \theta_r} f^c(\theta_n)\\
    &  + \left(y^c-f^c(\theta_n)\right)'\bpiInv\R\dmat\left(\nabla_{\theta} (\frac{\partial}{\partial \theta_r} f^c(\theta_n))(\hat{\theta}_n-\theta_n)\right)\\
    & + \left(y^c-f^c(\theta)\right)'\bpiInv\R\Ome \left( \frac{\partial}{\partial \theta_r} f^c(\hat{\theta}_n)- \frac{\partial}{\partial \theta_r} f^c(\theta_n)-\nabla_{\theta}\frac{\partial}{\partial \theta_r} f^c(\hat{\theta}_n)(\hat{\theta}_n-\theta_n)\right)\\
    & +\left(f^c(\theta_n)-f^c(\hat{\theta}_n)\right)'\bpiInv\R\Ome \left( \frac{\partial}{\partial \theta_r} f^c(\hat{\theta}_n)-  \frac{\partial}{\partial \theta_r} f^c(\theta_n)\right)\\
    =&-\left(\nabla_{\theta} f^c(\theta_n)(\hat{\theta}_n-\theta_n)\right)'\bpiInv\R\Ome \frac{\partial}{\partial \theta_r} f^c(\theta_n) \\
    & + \left(y^c-f^c(\theta_n)\right)'\bpiInv\R\Ome\left(\nabla_{\theta}(\frac{\partial}{\partial \theta_r} f^c(\theta_n))(\hat{\theta}_n-\theta_n)\right)\\
    & + O(\|\hat{\theta}_n-\theta_2\|_2^2)\\
     =& \sum_{r=1}^s  \frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)(\hat{\theta}_{n,t}-\theta_{n,t}) +O(\|\hat{\theta}_n-\theta_n\|_2^2),
\end{align*}
by the fact that $\viiii{\dmat}_1=O(1)$ and \ref{A:GMM2}. We note that the constant in $O(\|\hat{\theta}_n-\theta_n\|^2_2)$ is uniformly bounded above for all large $n$. 

Thus for term (A) we have:
\begin{align*}
    & \sum_{r=1}^s (\hat{g}_{n,r}(\hat{\theta}_n)-\hat{g}_{n,r}(\theta_n))\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)\\
    = & (\hat{\theta}_n-\theta_n)'\nabla_{\theta} \hat{g}_n(\theta_n)'\frac{\partial}{\partial \theta_t}\hat{g}_{n}(\theta_n) + O(\|\hat{\theta}_n-\theta_2\|_2^2),
\end{align*} where we also use the fact $\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)=O_p(1)$ by Lemma \ref{Lemma:bound}, Assumption \ref{A:GMM2}-(i) and the fact that $\viiii{\dmat}_1=O(1)$.
For term (B) we have:
\begin{equation*}
    o_p(1)\times O(\|\hat{\theta}_n-\theta_n\|_2)=o_p(\|\hat{\theta}_n-\theta_n\|_2),
\end{equation*}
where we use the fact that $\hat{g}_{n,r}(\theta_n)=\hat{g}_{n,r}(\theta_n)-g_{n,r}(\theta_n)+g_{n,r}(\theta_n)=o_p(1)+0$. Term (C) is of order $O(\|\hat{\theta}_n-\theta_n\|_2^2)$. 
To summarize, for the $t$th row of the equalities in equation (\ref{eq:25}), we have:
\begin{align*}
    0 = & \sum_{r=1}^s \hat{g}_{n,r}(\theta_n)\frac{\partial}{\partial \theta_t}\hat{g}_{n,r}(\theta_n)
    +  (\hat{\theta}_n-\theta_n)'\nabla \hat{g}_n(\theta_n)'\frac{\partial}{\partial \theta_t}\hat{g}_{n}(\theta_n) + o_p\left(\|\hat{\theta}_n-\theta_2\|_2\right) 
\end{align*}
Stacking the rows together we have the expression:
\begin{align*}
    0= & \nabla_{\theta} \hat{g}_{n}(\theta_n)'\hat{g}_n(\theta_n) + \nabla_{\theta} \hat{g}(\theta_n)'  \nabla_{\theta} \hat{g}(\theta_n) (\hat{\theta}_n-\hat{\theta}) + o_p(\|\hat{\theta}_n-\theta_n\|_2)
\end{align*}
Thus we have:
\begin{align*}
    &\hat{\theta}_n-\theta_n =  O_p\left( \left(\nabla_{\theta} \hat{g}_n(\theta_n)'  \nabla_{\theta} \hat{g}_n(\theta_n)\right)^{-1}\nabla_{\theta} \hat{g}_{n}(\theta_n)'\hat{g}_n(\theta_n)\right)
\end{align*}
Note $\nabla_{\theta} \hat{g}_n(\theta_n)-\nabla_{\theta} g_n(\theta_n) = o_p(1)$ by Lemma \ref{Lemma:bound}, Assumption \ref{A:GMM2}-(i) and the fact that $\viiii{\dmat}_1=O(1)$, and $\nabla_{\theta} \hat{g}_{n}(\theta_n)=O_p(1)$ as well. By Assumption \ref{A:GMM2}-(iv), $(\nabla_{\theta} \hat{g}_n(\theta_n)'  \nabla_{\theta} \hat{g}_n(\theta_n))^{-1}$ is  $O_p(1)$.  Thus
\begin{equation*}
    \hat{\theta}_n-\theta_n = O_p\left(\hat{g}_n\left(\theta_n\right)\right).
\end{equation*}
Since we have $g_n(\theta_n)=0$ by definition, then 
\begin{equation*}
       \hat{\theta}_n-\theta_n = O_p\left(\sqrt{\frac{\viiii{\dmat}_1^2\sigma_{\max}(\dmat)}{n}}\right) = O_p\left(\frac{1}{\sqrt{n}}\right)
\end{equation*}
by Lemma \ref{Lemma:bound} and that $\viiii{\dmat}_1=O(1)$. Rest proofs are similar to those in Theorem \ref{Thm:QMLE}.

%%%OLD REGULARITY CONDITIONS%%%%
\begin{assumption}\label{A:GMM2} Let $\theta_n$ be defined in Assumption \ref{A:GMM1}. Let $N$ be a positive integer.  Uniformly for all $n\geq N$, the following conditions are satisfied:
\begin{enumerate}[label=(\roman*)] 
\item (Moments)
\begin{enumerate}
   \item (Criterion Moments) For all $\theta\in\Theta$, there exists a $C_{\ref{A:GMM2},1}$ such that $\frac{1}{n}\sum_{a,i} \left( y_{ai}-f^a(x_i,\theta)\right)^4<C_{\ref{A:GMM2},1}$.
    \item (Derivative Moments) For all $\theta\in\Theta$,  there exists a $C_{\ref{A:GMM2},2}$ such that $\frac{1}{n}\sum_{a,i}\left(\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)\right)^4\leq C_{\ref{A:GMM2},2}$ and  $\frac{1}{n}\sum_{a,i}\left(\frac{\partial^2}{\partial \theta_t\partial \theta_u}f^a(x_i,\theta)\right)^4\leq C_{\ref{A:GMM2},2}$ for all $t,u\in [s]$.
\end{enumerate}
    \item  (Lipschitz Continuity for the Function and Its Derivatives) For all $a\in [k]$.
\begin{enumerate}
    \item  $f^a(x_i,\theta)$ is two-times differentiable in $\theta$ for all $x_i$, $i\in [n]$.
    \item  (Function) For all $\theta_1,\theta_2\in\Theta$, $|f^a(x_i,\theta_2)-f^a(x_i,\theta_1)|\leq D^{a}_{\ref{A:GMM2},3}(x_i)\|\theta_2-\theta_1\|_2$. There exists a $C_{\ref{A:GMM2},3}$ such that $\frac{1}{n}\sum_{a,i} (D^{a}_{\ref{A:GMM2},3}(x_i))^2<C_{\ref{A:GMM2},3}$.
     \item (First Derivatives)  For all $\theta_1,\theta_2\in\Theta$, $|\frac{\partial}{\partial \theta_t}f^a(x_i,\theta_2)- \frac{\partial}{\partial \theta_t}f^a(x_i,\theta_1)|\leq D^{a}_{\ref{A:GMM2},4}(x_i) \|\theta_2-\theta_1\|_2$ for all $k\in [s]$. There exists a $C_{\ref{A:GMM2},4}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},4}(x_i))^2 \leq C_{\ref{A:GMM2},4}$. 
     \item (Second Derivatives) There exists a $\epsilon$ such that for all $\theta\in B(\theta_n,\epsilon)$,  $|\frac{\partial^2}{\partial \theta_t\partial \theta_u}f^a(x_i,\theta)- \frac{\partial^2}{\partial \theta_t\partial \theta_u}f^a(x_i,\theta_n)|\leq D^{a}_{\ref{A:GMM2},5}(x_i) \|\theta-\theta_n\|_2$ for all $t,u\in [s]$. There exists a $C_{\ref{A:GMM2},5}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},5}(x_i))^2 \leq C_{\ref{A:GMM2},5}$. 
\end{enumerate}    
    \item (Taylor Approximations) For all $a\in [k]$,
\begin{enumerate}
    \item (First-Order Approximation for the Function) There exists an $\epsilon$ such that for all $\theta\in B(\theta_n,\epsilon)$,,  $|f^a(x_i,\theta)- f^a(x_i,\theta_n)-\nabla_{\theta}f^a(x_i,\theta_n)'(\theta-\theta_n)|\leq D^{a}_{\ref{A:GMM2},6}(x_i) \|\theta-\theta_n\|^2_2$ for all $t\in [s]$.   $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},6}(x_i))^2 \leq C_{\ref{A:GMM2},6}$.
    \item (First-Order Approximation for the First Derivative) There exists an $\epsilon$ such that for all $\theta\in B(\theta_n,\epsilon)$,  $|\frac{\partial}{\partial \theta_t}f^a(x_i,\theta)- \frac{\partial}{\partial \theta_t}f^a(x_i,\theta_n)-\nabla_{\theta} (\frac{\partial}{\partial \theta_t}f^a(x_i,\theta_n))'(\theta-\theta_n)|\leq D^{a}_{\ref{A:GMM2},7}(x_i) \|\theta-\theta_n\|^2_2$ for all $t\in [s]$. There exists a $C_{\ref{A:GMM2},7}$ such that $\frac{1}{n}\sum_{a,i}(D^{a}_{\ref{A:GMM2},7}(x_i))^2 \leq C_{\ref{A:GMM2},7}$.
\end{enumerate}
\item There exists a positive scalar $\epsilon$ such that the smallest absolute eigenvalue of the matrix \\$d g_n(\theta_n)\in \mathbb{R}^{s\times s}$  is greater than $\epsilon$, where $d g_n(\theta_n)$ is the differential of $g_n$ evaluated at $\theta_n$.   
\end{enumerate}
\end{assumption}
\begin{remark}
Assumption \ref{A:GMM2} can be checked by a Taylor expansion of the imputation functions coupled with appropriate moment conditions. 
\begin{comment}
2) Always inspect the eigenvalues of $\X'\Ome\X$; if the eigenvalues are very close to zero, try removing some covariate columns;  3) One could add some penalty terms onto the criterion, for example $\mathcal{L}_n(\theta)+\|\theta\|^2_2$. Solution to this problem is no longer optimal. However, one may gain identification and improved finite-sample performance in exchange for a loss of efficiency.
\end{comment}
\end{remark}
